Scoring with Large Language Models: A Study on Measuring Empathy of Responses in Dialogues

In recent years, Large Language Models (LLMs) have become increasingly more powerful in their ability to complete complex tasks. One such task in which LLMs are often employed is scoring, i.e., assigning a numerical value from a certain scale to a subject. In this paper, we strive to understand how LLMs score, specifically in the context of empathy scoring. We develop a novel and comprehensive framework for investigating how effective LLMs are at measuring and scoring empathy of responses in dialogues, and what methods can be employed to deepen our understanding of LLM scoring. Our strategy is to approximate the performance of state-of-the-art and fine-tuned LLMs with explicit and explainable features. We train classifiers using various features of dialogues including embeddings, the Motivational Interviewing Treatment Integrity (MITI) Code, a set of explicit subfactors of empathy as proposed by LLMs, and a combination of the MITI Code and the explicit subfactors. Our results show that when only using embeddings, it is possible to achieve performance close to that of generic LLMs, and when utilizing the MITI Code and explicit subfactors scored by an LLM, the trained classifiers can closely match the performance of fine-tuned LLMs. We employ feature selection methods to derive the most crucial features in the process of empathy scoring. Our work provides a new perspective toward understanding LLM empathy scoring and helps the LLM community explore the potential of LLM scoring in social science studies.

==> backup.tex <==
%
\begin{comment}
\begin{table}[htbp]
\caption{Scoring Accuracy of Different GPT Models} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf Model} & {\bf Fine-Tune Parameters} & {\bf Accuracy}  \\
\hline
gpt-3.5-turbo & N/A & {\bf 0.3854} \\
\hline
gpt-4 & N/A & 0.4375 \\
\hline
gpt-4o & N/A & 0.3880 \\
\hline
gpt-4o-mini & N/A & {\bf 0.4661} \\
\hline
gpt-4o-mini & Epoch: 3; Learning\_rate\_multiplier: 1.8 & 0.4844 \\
\hline
gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.25 & 0.5417 \\
\hline
gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.5 & {\bf 0.5469} \\
\hline
gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.75 & 0.5365 \\
\hline
gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 1 & 0.5130 \\
\hline
\end{tabular}
\label{tab:models}
\end{center}
% \vspace{-20pt}
\end{table}
%
\end{comment}


% \begin{table}[htbp]
% \centering
% \small % This command will make the font smaller
% \caption{Accuracy on different LLMs.}
% \begin{tabular}{crrr}
% \toprule

% {\bf Model} & {\bf Accuracy}  \\
% \midrule
% gpt-3.5-turbo & {\bf 0.3854} \\

% gpt-4 & 0.4375 \\

% gpt-4o & 0.3880 \\

% gpt-4o-mini & {\bf 0.4661} \\
% \bottomrule
% \end{tabular}
% \label{tab:models}

% % \vspace{-20pt}
% \end{table}
%





% However, our study’s main focus is to understand how the LLMs measure and score empathy. To do this, we use several different methods of “subfactorization” and regression/classifier model training to achieve similar accuracy to the baseline accuracy and also attempt to reach the peak accuracy obtained through fine-tuning.



% \begin{table}[htbp]
% \caption{Scoring Accuracy of Fine-Tuned GPT-4o-mini Utilizing Different Parameters} 
% \centering
% \small % This command will make the font smaller
% \begin{tabular}{crrr}
% \toprule

% {\bf Model} & {\bf Fine-Tune Parameters} & {\bf Accuracy}  \\
% \midrule
% gpt-4o-mini & Epoch: 3; Learning\_rate\_multiplier: 1.8 & 0.4844 \\

% gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.25 & 0.5417 \\

% gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.5 & {\bf 0.5469} \\

% gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 0.75 & 0.5365 \\

% gpt-4o-mini & Epoch: 4; Learning\_rate\_multiplier: 1 & 0.5130 \\
% \bottomrule
% \end{tabular}
% \label{tab:fine-tune-models}

% % \vspace{-20pt}
% \end{table}

\begin{comment}
\begin{table}[htbp]
\caption{Scoring Accuracy of Various Regression Models on 15 Subfactors V2} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf Model} & {\bf Accuracy}  \\
\hline
Logistic Regression & 0.4948 \\
\hline
SVC & 0.5130 \\ 
\hline
Decision Tree & 0.4010 \\
\hline
Random Forrest & 0.4427 \\
\hline
MLP & 0.4323 \\
\hline
\end{tabular}
\label{tab:15v2}
\end{center}
\end{table}
\end{comment}


% This gave hints that maybe feature selection can help improve the results. 

\begin{comment}
\begin{table}[htbp]
\caption{Scoring Accuracy of Various Regression Models on 15 Subfactors V2 + Miti Code without feature selection} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf Model} & {\bf Accuracy}  \\
\hline
Logistic Regression & 0.4948 \\
\hline
SVC & 0.5 \\ 
\hline
Decision Tree & 0.3802 \\
\hline
Random Forrest & 0.4479 \\
\hline
MLP & 0.4271 \\
\hline
\end{tabular}
\label{tab:15v2-miti}
\end{center}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[htbp]
\caption{Importance of Different Features} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf \#} &                   {\bf Feature} & {\bf Importance} \\
\hline
25 &                              Confront & 0.445108 \\
\hline
27 &                                  Warn & 0.410316 \\
\hline
26 &                                Direct & 0.395612 \\
\hline
20 &                Advise with Permission & 0.383294 \\
\hline
23 &                               Support & 0.273697 \\
\hline
22 &                    Emphasize Autonomy & 0.216146 \\
\hline
8  &               validation of feelings  &  0.179611 \\
\hline
29 &                                Other  &  0.174904 \\
\hline
10 &                        encouragement  &  0.174515 \\
\hline
15 &                      Closed Question  &  0.150571 \\
\hline
16 &                        Open Question  &  0.132135 \\
\hline
13 &                           empowering  &  0.121820 \\
\hline
11 &                          reassurance  &  0.121385 \\
\hline
4  &                  clarity of response  &  0.120640 \\
\hline
28 &                        Self Disclose  &  0.110452 \\
\hline
5  &                       warmth in tone  &  0.103984 \\
\hline
9  &                  emotional resonance  &  0.098530 \\
\hline
21 &                               Affirm  &  0.085976 \\
\hline
12 &                        offering help  &  0.062364 \\
\hline
24 &            Advise without Permission  &  0.052836 \\
\hline
18 &                   Complex Reflection  &  0.050148 \\
\hline
0  &                   perspective taking  &  0.044418 \\
\hline
2  &                 contextual awareness  &  0.044396 \\
\hline
14 &                           assistance  &  0.042678 \\
\hline
3  & acknowledgment of speaker's experience  &  0.040109 \\
\hline
17 &                    Simple Reflection  &  0.031139 \\
\hline
19 &                     Give Information  &  0.016307 \\
\hline
6  &                sympathetic responses  &  0.013130 \\
\hline
1  &              recognition of emotions  &  0.011837 \\
\hline
7  &                  emotional-mirroring  &  0.002526 \\
\hline
\end{tabular}
\label{tab:feature-importlance}
\end{center}
\end{table}
\end{comment}

% \begin{wraptable}{r}{0.55\columnwidth}
% \vspace{-5mm}
% \caption{Scoring Accuracy of Various Classifiers on Embeddings}
% \centering
% \small % This command will make the font smaller
% \begin{tabular}{cr}
% \toprule
% {\bf Model} & {\bf Accuracy}  \\
% \midrule
% Logistic Regression & 0.4193 \\
% SVC & 0.4271 \\
% Decision Tree & 0.3984 \\
% Random Forrest & 0.4063 \\
% MLP  & 0.4219 \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:embeddings}
% \end{wraptable}

\begin{comment}
\begin{table}[htbp]
\caption{Scoring Accuracy of Various Regressors on Embeddings} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf Model} & {\bf Accuracy}  \\
\hline
Logistic Regression & 0.4193 \\
\hline
SVC & 0.4271 \\
\hline
Decision Tree & 0.3984 \\
\hline
Random Forrest & 0.4063 \\
\hline
MLP  & 0.4219 \\
\hline
\end{tabular}
\label{tab:embeddings}
\end{center}
\end{table}
\end{comment}

% \begin{figure}[htbp]
% % \centerline{\includegraphics[width=0.9\columnwidth]{figures/Table2Graph.svg}}
% \centerline{\includesvg[width=0.9\columnwidth]{figures/Fig1.svg}}
% \caption{Scoring Accuracy of Various Classifiers on Embeddings}
% \label{fig1}
% \end{figure}

% \begin{wraptable}{r}{0.55\columnwidth}
% % \vspace{-5mm}
% \caption{Scoring Accuracy of Various Classifiers on MITI Code}
% \centering
% \small % This command will make the font smaller
% \begin{tabular}{cr}
% \toprule
% {\bf Model} & {\bf Accuracy}  \\
% \midrule
% Logistic Regression & 0.4401 \\
% SVC & 0.4479 \\ 
% Decision Tree & 0.4089 \\
% Random Forrest & 0.4167 \\
% MLP & 0.4141 \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:miti}
% \end{wraptable}

\begin{comment}
\begin{table}[htbp]
\caption{Scoring Accuracy of Various Regression Models on the Miti Code} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf Model} & {\bf Accuracy}  \\
\hline
Logistic Regression & 0.4401 \\
\hline
SVC & 0.4479 \\ 
\hline
Decision Tree & 0.4089 \\
\hline
Random Forrest & 0.4167 \\
\hline
MLP & 0.4141 \\
\hline
\end{tabular}
\label{tab:miti}
\end{center}
\end{table}
\end{comment}

% \begin{figure}[htbp]
% % \centerline{\includegraphics[width=\columnwidth]{figures/TableIIIGraph.png}}
% \centerline{\includesvg[width=0.9\columnwidth]{figures/Fig2.svg}}
% \caption{Scoring Accuracy of Various Classifiers on MITI Code}
% \label{fig2}
% \end{figure}

% \begin{table}[htbp]
% \caption{Regression Models Utilized in this Study}
% \begin{center}
% \begin{tabular}{|l|r|}
% \hline
% {\bf Regression Models} \\
% \hline
% Linear Regression \\
% Polynomial Regression \\
% Decision Tree Regressor \\
% Random Forest Regressor \\
% Support Vector Regression \\
% Ada Boost Regressor \\
% Bagging Regressor \\
% Extra Trees Regressor \\
% Gradient Boosting Regressor \\
% Stacking Regressor \\
% Simple Neural Network \\
% \hline
% \end{tabular}
% \label{tab:regressionmodels}
% \end{center}
% \end{table}

% \begin{table}[htbp]
% \caption{3 Dimensions of Empathy and Their Subfactors (Second Set)} 
% \begin{center}
% \begin{tabular}{|l|r|}
% \hline
% {\bf Dimension}       & {\bf Subfactor}  \\
% \hline
% Cognitive Empathy     & Perspective Taking \\
%                       & Recognition of Emotions \\
%                       & Contextual Awareness \\
%                       & Acknowledgment of Speaker's Experience \\
%                       & Clarity of Response \\
% \hline
% Affective Empathy     & Warmth in Tone \\
%                       & Sympathetic Responses \\
%                       & Emotional Mirroring \\
%                       & Validation of Feelings \\
%                       & Emotional Resonance \\
% \hline
% Compassionate Empathy & Encouragement \\
%                       & Reassurance \\
%                       & Offering Help \\
%                       & Empowering \\
%                       & Assistance \\
% \hline
% \end{tabular}
% \label{tab:subfactors}
% \end{center}
% \end{table}


 


% \begin{table}[htbp]
% \caption{Scoring Accuracy of Different Prompt Combinations}
% \centering
% \small % This command will make the font smaller
% \begin{center}
% \begin{tabular}{crrr}
% \toprule


% {\bf Model} & {\bf Prompts} & {\bf Accuracy}  \\
% \midrule
% gpt-4o-mini & Naive & 0.4661 \\
% % \hline
% % gpt-4o-mini & Naive + 3 Dims & 0.4844 \\

% gpt-4o-mini & Naive + 3 Dims + 15 Subfactors V1 & 0.4818 \\

% gpt-4o-mini & Naive + 3 Dims + 15 Subfactors V2 & {\bf 0.4844} \\
% \bottomrule
% \end{tabular}
% \label{tab:prompt-accuracies}
% \end{center}
% %\vspace{-20pt}
% \end{table}

% \begin{wraptable}{r}{0.55\columnwidth}
% % \vspace{-5mm}
% \caption{Scoring Accuracy of Various Classifiers on 15 Subfactors V2}
% \centering
% \small % This command will make the font smaller
% \begin{tabular}{cr}
% \toprule
% {\bf Model} & {\bf Accuracy}  \\
% \midrule
% Logistic Regression	& 0.4948 \\
% SVC	& 0.5130 \\
% Decision Tree	& 0.4010 \\
% Random Forest	& 0.4427 \\
% MLP	& 0.4323 \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \label{tab:subfactors}
% \end{wraptable}

% \begin{figure}[htbp]
% \vspace{-10pt}
% % \centerline{\includegraphics[width=\columnwidth]{figures/TableIVGraph.png}}
% \centerline{\includesvg[width=0.9\columnwidth]{figures/Fig3.svg}}
% \caption{Scoring Accuracy of Classifiers on 15 Subfactors V2}
% \label{fig3}
% \vspace{-10pt}
% \end{figure}

% \begin{figure}[htbp]
% % \centerline{\includegraphics[width=\columnwidth]{figures/TableVGraph.png}}
% % \centerline{\includesvg[width=\columnwidth]{figures/Fig4.svg}}
% \centerline{\includesvg[width=0.95\columnwidth]{figures/15v2-MITI-Accuracy-Comp.svg}}
% \caption{Accuracy of Regression Models on 15 Subfactors V2 + MITI Code}
% \label{fig:subfactors-miti}
% \end{figure}

% \begin{figure}[htbp]
% \vspace{-7mm}
% \centerline{\includesvg[width=0.9\columnwidth]{figures/15v2-MITI-RFE.svg}}
% \caption{Feature Selection with RFE}
% \label{fig5}
% \vspace{-5pt}
% \end{figure}

% \begin{figure}[htbp]
% % \vspace{-7mm}
% \vspace{-10pt}
% \centerline{\includesvg[width=0.9\columnwidth]{figures/15v2-MITI-Feature-Importance.svg}}
% \caption{Feature Importance}
% \label{fig6}
% %\vspace{-10pt}
% \end{figure}




%\subsection{Integrating Feature Selection}

\begin{comment}
\begin{figure}[htbp]
\caption{Importance of Different Features}
\centerline{\includesvg[width=\columnwidth]{figures/Fig5.svg}}
\label{fig5}
\vspace{-30pt}
\end{figure}
\end{comment}

% To be able to further improve the performance of our trained classifiers, we employed the K-Best and RFE feature selection algorithms. The feature space consists of 15 MITI features and 15 explicit subfactors.
% The selected feature number ranges from 1 to 30. We used the Linear Regression Classifier as our example model. Running the RFE algorithm selecting $k$ features, where $k$ is within the range described above, the best number of features to select on the combination of the MITI Code and 15 subfactors, the best number of features was 10 features, producing a slightly higher accuracy of 53.65\% accuracy, as shown in Figure \ref{fig6}. The K-Best algorithm is less effective in this task because it achieves the highest performance when selecting 1 feature. The importance of each feature (generated by the Linear Regression Classifier), which measures how much a feature contributes to model training, can be found in Figure~\ref{fig5}, where the capitalized features are part of the MITI Code while the lower case features are part of the 15 subfactors V2 set. We use this classifier model as an example of what the performance of feature selection + MITI Code + 15 subfactors can achieve. The results from RFE selection show that when selecting the most optimal set of features from the set of MITI Code and 15 subfactors for classifier training, the performance of the classifiers can reach close to the peak performance of the fine-tuned GPT-4o-mini model, and there is an increase in accuracy when compared to training classifiers without feature selection. 

\begin{comment}
\begin{table}[htbp]
\caption{Feature selection with KBest and RFE} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf \# of Feature Selected} & {\bf KBest} & {\bf RFE} \\
\hline
1 & 0.5026041667  & 0.3307291667 \\
\hline
2 & 0.4869791667  & 0.3697916667 \\
\hline
3 & 0.4609375     & 0.4713541667 \\
\hline
4 & 0.4375        & 0.4713541667 \\
\hline
5 & 0.3880208333  & 0.4661458333 \\
\hline
6 & 0.4427083333  & 0.4557291667 \\
\hline
7 & 0.4036458333  & 0.4739583333 \\
\hline
8 & 0.4296875	  & 0.4739583333 \\
\hline
9 & 0.4166666667  & 0.4765625 \\
\hline
10 & 0.4166666667 & {\bf 0.5364583333} \\ 
\hline
11 & 0.40625	  & 0.5286458333 \\ 
\hline
12 & 0.4192708333 & 0.5104166667 \\
\hline
13 & 0.4453125	  & 0.5286458333 \\
\hline
14 & 0.4348958333 & 0.5130208333 \\
\hline
15 & 0.4583333333 & 0.5078125 \\
\hline
\end{tabular}
\label{tab:feature-selection}
\end{center}
\end{table}
\end{comment}

% \begin{figure}[htbp]
% \caption{Scoring Accuracy of Regression Models on 15 Subfactors V2 + MITI Code with K-Best and RFE Feature Selection}
% \centerline{\includesvg[width=\columnwidth]{figures/Fig6.svg}}
% \label{fig6}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/3D_Accuracy_Plot.pdf}
%     \caption{Scoring Accuracy of Regression Models on 15 Subfactors V2 + MITI Code with K-Best and RFE Feature Selection}
%     \label{fig6}
% \end{figure}

% \title{\hspace{-0.15in} Scoring with Large Language Models: A Study on Measuring Empathy of Responses in Dialogues
% }

